Comprehensive Analysis of Negative Sampling in Knowledge Graph Representation Learning

Negative sampling (NS) loss plays an important role in learning knowledge graph embedding (KGE) to handle a huge number of entities. However, the performance of KGE degrades without hyperparameters such as the margin term and number of negative samples in NS loss being appropriately selected. Currently, empirical hyperparameter tuning addresses this problem at the cost of computational time. To solve this problem, we theoretically analyzed NS loss to assist hyperparameter tuning and understand the better use of the NS loss in KGE learning. Our theoretical analysis showed that scoring methods with restricted value ranges, such as TransE and RotatE, require appropriate adjustment of the margin term or the number of negative samples different from those without restricted value ranges, such as RESCAL, ComplEx, and DistMult. We also propose subsampling methods specialized for the NS loss in KGE studied from a theoretical aspect. Our empirical analysis on the FB15k-237, WN18RR, and YAGO3-10 datasets showed that the results of actually trained models agree with our theoretical findings.

==> conclusion.tex <==
In this paper, we conducted a theoretical analysis for the NS loss used in KGE learning and derived some theoretical facts.
Based on the theoretical facts, we also proposed subsampling methods suitable for the NS loss function of KGE learning. In order to verify the validity of these theoretical facts and the performance of the proposed subsampling method, we conducted experiments on FB15k-237, WN18RR, and YAGO3-10 datasets. 
The experimental results show that the theoretical facts we derived are also observed in the real-world datasets. We also show that the proposed subsampling methods can improve the KGC performance consistently.
